Unify and Triumph: Polyglot, Diverse, and Self-Consistent Generation of Unit Tests with LLMs

Large language model (LLM)-based test generation has gained attention in software engineering, yet most studies evaluate LLMs' ability to generate unit tests in a single attempt for a given language, missing the opportunity to leverage LLM diversity for more robust testing. This paper introduces PolyTest, a novel approach that enhances test generation by exploiting polyglot and temperature-controlled diversity. PolyTest systematically leverages these properties in two complementary ways: (1) Cross-lingual test generation, where tests are generated in multiple languages at zero temperature and then unified; (2) Diverse test sampling, where multiple test sets are generated within the same language at a higher temperature before unification. A key insight is that LLMs can generate diverse yet contradicting tests -- same input, different expected outputs -- across languages and generations. PolyTest mitigates inconsistencies by unifying test sets, fostering self-consistency and improving overall test quality. Unlike single-language or single-attempt approaches, PolyTest enhances testing without requiring on-the-fly execution, making it particularly beneficial for weaker-performing languages. We evaluate PolyTest on Llama3-70B, GPT-4o, and GPT-3.5 using EvalPlus, generating tests in five languages (Java, C, Python, JavaScript, and a CSV-based format) at temperature 0 and sampling multiple sets at temperature 1. We observe that LLMs frequently generate contradicting tests across settings, and that PolyTest significantly improves test quality across all considered metrics -- number of tests, passing rate, statement/branch coverage (up to +9.01%), and mutation score (up to +11.23%). Finally, PolyTest outperforms Pynguin in test generation, passing rate, and mutation score.

==> bigTableComparaison.tex <==

\begin{table*}
        
        \caption{Average of statement coverage, branch coverage, and mutation score.}
        \label{table:coverageMutation}
        %\hspace*{-0.5cm}
        \resizebox{0.7\textwidth}{!} {
        \begin{tabular}{lllccc}
        \toprule
        \centering
        LLM & Language & Step & Statement coverage & Branch coverage & Mutation score \\ \midrule

        &   & Gen. & 87.93\% & 85.63\% & 70.54\% \\ 
        &  C & Ampl. & 87.37\% & 85.61\% & 71.05\% \\
        &   & Redu. & 87.94\% & 85.27\% & 67.63\% \\ \cmidrule{2-6}

         &  & Gen. & 85.98\% & 83.85\% & 68.12\%  \\ 
        &  CSV & Ampl. & 87.93\% & 86.24\% & 72.30\%   \\
         &  & Redu. & 84.21\% & 81.07\% & 64.19\% \\ \cmidrule{2-6}

          &   & Gen. & 93.80\% & 92.17\% & 76.38\% \\ 
       \emph{llama3-70b} &  Java & Ampl. & 95.05\% & 93.87\% & 78.61\% \\
        &   & Redu. & 92.32\% & 89.68\% & 71.10\% \\ \cmidrule{2-6}

         &   & Gen. & 93.27\% & 91.76\% & 76.03\% \\ 
        &  Javascript & Ampl. & 93.78\% & 92.64\% & 78.16\% \\
        &   & Redu. & 91.34\% & 88.74\% & 71.43\% \\ \cmidrule{2-6}

       &  & Gen. & 97.68\% & 96.79\% & 82.68\% \\ 
        &  Python & Ampl. & 98.75\% & 98.03\% & 83.42\% \\
        &   & Redu. & 95.57\% & 93.59\% & 76.56\% \\ \cmidrule{2-6}

%&  Python & Ampl. & 98.75\% & 98.03\% & 83.42\% \\

         &  & Gen. & 99.37\% \cellcolor{green!35}& 98.65\% \cellcolor{green!35}& 84.85\% \cellcolor{green!35} \\ 
       &   \polytest & Ampl. & 99.48\% \cellcolor{green!35}& 98.87\% \cellcolor{green!35}& 85.73\% \cellcolor{green!35} \\
        &   & Redu. & 97.23\% \cellcolor{green!35}& 95.56\% \cellcolor{green!35}& 78.36\% \cellcolor{green!35}\\  \midrule \midrule

%first	84.57 > 84.85121951 + 0.32
%amplified	85.76 > 85.72 - 0.04
%minimized	78.89 > 78.36380368 - 0.53


        &   & Gen. & 84.05\% & 80.73\% & 65.66\% \\ 
        &  C & Ampl. & 85.72\% & 82.37\% & 68.32\% \\ 
        &   & Redu. & 85.53\% & 81.94\% & 65.89\% \\  \cmidrule{2-6}
  
         &  & Gen. & 97.37\% & 95.49\% & 80.30\% \\ 
        &  CSV & Ampl. & 97.29\% & 95.93\% & 80.95\% \\ 
         &  & Redu. & 96.62\% & 94.75\% & 79.65\% \\  \cmidrule{2-6}

          &   & Gen. & 96.81\% & 94.76\% & 79.06\% \\ 
       \emph{GPT-3.5-turbo} &  Java & Ampl. & 96.84\% & 95.24\% & 81.55\% \\
        &   & Redu. & 97.41\% & 95.58\% & 80.44\% \\   \cmidrule{2-6}

         &   & Gen. & 95.75\% & 93.87\% & 78.72\% \\
        &  Javascript & Ampl. & 96.17\% & 94.57\% & 80.83\% \\
        &   & Redu. & 96.31\% & 94.60\% & 79\% \\  \cmidrule{2-6}

       &  & Gen. & 95.83\% & 94.04\% & 78.28\% \\ 
        &  Python & Ampl. & 97.13\% & 95.46\% & 80.26\% \\ 
        &   & Redu. & 96.48\% & 94.76\% & 80.14\% \\  \cmidrule{2-6}

         &  & Gen. & 98.48\% \cellcolor{green!35} & 96.85\% \cellcolor{green!35} & 81.91\% \cellcolor{green!35} \\ 
       &   \polytest & Ampl. & 98.89\% \cellcolor{green!35} & 97.84\% \cellcolor{green!35} & 85.6\% \cellcolor{green!35} \\ 
        &   & Redu. & 97.90\% \cellcolor{green!35} & 96.41\% \cellcolor{green!35} & 82\% \cellcolor{green!35} \\   \bottomrule 

        \end{tabular}
    }
\end{table*}

==> bigTableComparaisonMultipleGen.tex <==

\begin{table*}
        
        \caption{Todo for new experiment. \red{Multiple generations at temp = 1 vs \polytest at temp = 0}} %Average of statement coverage, branch coverage, and mutation score.
        \label{table:coverageMutation}
        %\hspace*{-0.5cm}
        \resizebox{0.8\textwidth}{!} {
        \begin{tabular}{lll cc ccc}
        \toprule
        \centering
        LLM & Language & Step & \begin{tabular}[c]{@{}l@{}}$n^o$ of total \\ test \end{tabular}& \begin{tabular}[c]{@{}l@{}}$n^o$ of passing \\ tests\end{tabular} & \begin{tabular}[c]{@{}l@{}}Statement \\ coverage \end{tabular}& \begin{tabular}[c]{@{}l@{}}Branch \\ coverage\end{tabular} & \begin{tabular}[c]{@{}l@{}}Mutation \\ score\end{tabular} \\ \midrule


        &   & Gen. & 1736 & 1083 (62.38\%) &  86\% & 83.75\% & 70.54\% \\ 
        &  C & Ampl. & 3024 & 1813 (60\%) &  85.95\% & 83.65\% & 70.80\% \\ 
        &   & Redu. & 503 & 380 (75.55\%) &  89.16\% & 86.96\% & 70.70\% \\  \cmidrule{2-8}

         &  & Gen. & 2139 & 1544 (72.18\%) &  95.55\% & 94.64\% & 81.36\%  \\ 
        &  CSV & Ampl. & 3452 & 2477 (71.75\%) &  95.72\% & 94.72\% & 81.54\%  \\ 
         &  & Redu. & 529 & 455 (86\%) &  93.97\% & 92.53\% & 76.22\%  \\ \cmidrule{2-8}

          &   & Gen. & 1437 & 1098 (76.41\%) &  98.14\% & 97.37\% & 81.92\%  \\ 
       \emph{llama3} &  Java & Ampl. & 2452 & 1819 (74.18\%) &  98.57\% & 97.81\% & 85.80\%  \\  
       \emph{-70b} &   & Redu. & 433 & 396 (91.45\%) &  96.34\% & 94.48\% & 76.97\%  \\ \cmidrule{2-8}

         &   & Gen. & 1604 & 1231 (76.75\%) &  97.01\% & 96.06\% & 82.26\%  \\  
        &  Javascript & Ampl. & 2786 & 1965 (70.53\%) &  95.59\% & 94.33\% & 80.93\%  \\ 
        &   & Redu. & 458 & 417 (91.04\%) &   96.65\% & 94.76\% & 78.07\%  \\  \cmidrule{2-8}

       &  & Gen. & 1676 & 1339 (79.89\%) &   99.37\% & 98.72\% & 84.76\%  \\ 
        &  Python & Ampl. & 2804 & 2106 (75.10\%) &   98.93\% & 98.37\% & 85.14\%  \\ 
        &   & Redu. & 454 & 419 (92.29\%)&   96.50\% & 94.91\% & 78.13\%  \\  \cmidrule{2-8}

%&  Python & Ampl. & 98.75\% & 98.03\% & 83.42\% \\

         &  & Gen. & 2291 & 1528 (66.70\%) &  99.37\% \cellcolor{green!35}& 98.65\% \cellcolor{green!35}& 84.85\% \cellcolor{green!35} \\ 
       &   \polytest & Ampl. & 3663 & 2360 (64.43\%) &  99.48\% \cellcolor{green!35}& 98.87\% \cellcolor{green!35}& 85.73\% \cellcolor{green!35} \\
        &   & Redu. & 689 & 524 (76\%) &  97.23\% \cellcolor{green!35}& 95.56\% \cellcolor{green!35}& 78.36\% \cellcolor{green!35}\\  \midrule \midrule

%first	84.57 > 84.85121951 + 0.32
%amplified	85.76 > 85.72 - 0.04
%minimized	78.89 > 78.36380368 - 0.53

        &   & Gen. & ? & ? &   \% & \% & \%  \\ 
        &  C & Ampl. &  ? & ? &  \% & \% & \%  \\ 
        &   & Redu. & ? & ? &   \% & \% & \%  \\ \cmidrule{2-8}
  
         &  & Gen. &  ? & ? &  \% & \% & \%  \\ 
        &  CSV & Ampl. & ? & ? &   \% & \% & \%  \\ 
         &  & Redu. & ? & ? &   \% & \% & \%  \\ \cmidrule{2-8}

          &   & Gen. & ? & ? &  \% & \% & \%  \\ 
       \emph{GPT-3.5} &  Java & Ampl. &  ? & ? &  \% & \% & \%  \\ 
       \emph{-turbo} &   & Redu. & ? & ? &  \% & \% & \%  \\   \cmidrule{2-8}

         &   & Gen. &  ? & ? &  \% & \% & \%  \\ 
        &  Javascript & Ampl. &  ? & ? &   \% & \% & \%  \\ 
        &   & Redu. &  ? & ? & \%  & \% & \%  \\  \cmidrule{2-8}

       &  & Gen. &  ? & ? &  \% & \% & \%  \\ 
        &  Python & Ampl. & ? & ? &  \% & \% & \%  \\ 
        &   & Redu. &  ? & ? &  \% & \% & \%  \\ \cmidrule{2-8}

         &  & Gen. &  689 & 521 (75.62\%) & 98.48\% \cellcolor{green!35} & 96.85\% \cellcolor{green!35} & 81.91\% \cellcolor{green!35} \\ 
       &   \polytest & Ampl. &  2003 & 1337 (66.75\%) & 98.89\% \cellcolor{green!35} & 97.84\% \cellcolor{green!35} & 85.6\% \cellcolor{green!35} \\ 
        &   & Redu. &  832 & 616 (74\%)  & 97.90\% \cellcolor{green!35} & 96.41\% \cellcolor{green!35} & 82\% \cellcolor{green!35} \\   \bottomrule 

        \end{tabular}
    }
\end{table*}

==> temp_metadata.tex <==

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>00000000.0000000.0000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>00000000.00000000.00000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>00000000.00000000.00000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>00000000.00000000.00000000</concept_id>
  <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc[300]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc{Do Not Use This Code~Generate the Correct Terms for Your Paper}
\ccsdesc[100]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
